Open-Source CubeSat Solar Panels: Design, Assembly, Testing, and On-Orbit Demonstration

Cube satellites, or CubeSats, are small satellites commonly used to perform Earth imaging and on-orbit scientific experiments. CubeSats are often powered using expensive, inflexible commercial-off-the-shelf solar panels, largely due to a lack of flight-qualified open-source alternatives. Here, we describe the design of customizable, deployable solar panels, offering an open-source, cost-effective alternative. Towards a fully open-source CubeSat, our designs have mission-tailored power generation capabilities and simple electrical and mechanical integration. The solar panel designs were demonstrated on-orbit on three satellites in the Northern SPIRIT constellation and will be on AlbertaSat's Ex-Alta~3 satellite, which will launch in 2025. The design files, assembly procedures, and best practices will be open-source-published online. This work lowers the barrier of entry into space, making satellite design easier and less expensive -- students helping students design better satellites.

==> content/articleFrontMatterDrafting.tex <==
\renewcommand{\maketitlehookd}{
    \begin{abstract} 
    \abstractText
    \end{abstract}
}

\title{\doctitle}
\author{\authors}
\date{\small\textit{\addressOne \\ \addressTwo \\ \emailContact}}

\maketitle
